Multi-level Convolutional Autoencoder Networks for Parametric Prediction of Spatio-temporal Dynamics

A data-driven framework is proposed towards the end of predictive modeling of complex spatio-temporal dynamics, leveraging nested non-linear manifolds. Three levels of neural networks are used, with the goal of predicting the future state of a system of interest in a parametric setting. A convolutional autoencoder is used as the top level to encode the high dimensional input data along spatial dimensions into a sequence of latent variables. A temporal convolutional autoencoder (TCAE) serves as the second level, which further encodes the output sequence from the first level along the temporal dimension, and outputs a set of latent variables that encapsulate the spatio-temporal evolution of the dynamics. The use of dilated temporal convolutions grows the receptive field exponentially with network depth, allowing for efficient processing of long temporal sequences typical of scientific computations. A fully-connected network is used as the third level to learn the mapping between these latent variables and the global parameters from training data, and predict them for new parameters. For future state predictions, the second level uses a temporal convolutional network to predict subsequent steps of the output sequence from the top level. Latent variables at the bottom-most level are decoded to obtain the dynamics in physical space at new global parameters and/or at a future time. Predictive capabilities are evaluated on a range of problems involving discontinuities, wave propagation, strong transients, and coherent structures. The sensitivity of the results to different modeling choices is assessed. The results suggest that given adequate data and careful training, effective data-driven predictive models can be constructed. Perspectives are provided on the present approach and its place in the landscape of model reduction.

==> nomenclature.tex <==
\section*{Nomenclature}
{\renewcommand\arraystretch{1.0}
\noindent\begin{longtable*}{@{}l @{\quad=\quad} l@{}}
{$\alpha$}&{Perturbation amplification factor on pressure}\\
{$\eta$}&{Learning rate}\\
{$\mathcal{L}$}&{Loss function}\\
{$q_s$}&{Code for convolutional }\\
{$\mu$}&{Global parameter}\\
{$\theta$}&{Inflow side-slip angle}\\
{$u$}&{Stream-wise velocity}\\
{$x$}&{Flow field data}\\


% \multicolumn{2}{@{}l}{Superscripts}\\
% {$l1(e/d)$}&{First-level - 2D/3D convolutional autoencoder (encoder/decoder)}\\
% {$l2(e/d)$}&{Second-level - Temporal convolutional autoencoder (encoder/decoder)}\\
% {$l3$}&{Third-level - Fully connected feedforward network}\\

% \multicolumn{2}{@{}l}{Subscripts}\\
% {train}&{Training}\\
% {test}&{Testing}\\

\end{longtable*}}
% \printnomenclature
